Enhance Feature Discrimination for Unsupervised Hashing

We introduce a novel approach to improve unsupervised hashing. Specifically, we propose a very efficient embedding method: Gaussian Mixture Model embedding (Gemb). The proposed method, using Gaussian Mixture Model, embeds feature vector into a low-dimensional vector and, simultaneously, enhances the discriminative property of features before passing them into hashing. Our experiment shows that the proposed method boosts the hashing performance of many state-of-the-art, e.g. Binary Autoencoder (BA) [1], Iterative Quantization (ITQ) [2], in standard evaluation metrics for the three main benchmark datasets.

==> tex/2-proposed_methods.tex <==
\section{Proposed method}
\label{sec:proposed_method}
In this section, we describe the details of the proposed method in three main steps. For the first step (Section \ref{ssec:proposed_method_dim_reduce}), we pre-process descriptors by Principal Component Analysis (PCA). The major novelty of our method is discussed in the second step (Section \ref{ssec:proposed_method_embedding}), in which we attempt to embedding data to lower-dimensional space and enhancing feature discrimination concurrently by utilizing the posterior probabilities of Gaussian Mixture Model (GMM). In the last step (Section \ref{ssec:proposed_method_unsparsifying}), the embedding features are post-processed by Power Normalization to make them more robust to $l2$-distance similarity \cite{PN_Perronnin:2010:IFK:1888089.1888101}. As a result, the compact and discriminative feature can be fed into any hashing methods to produce hashing code.

% \vspace{-1.5em}
\subsection{Dimension reduction}
\label{ssec:proposed_method_dim_reduce}
Given a set of $m$ high-dimensional data points
%\footnote{The data have been zero-centered.} 
- $\tilde{X}=\{\tilde{x}^{(1)}, \tilde{x}^{(2)}, ..., \tilde{x}^{(m)}\}; \tilde{x}^{(i)} \in \mathbb{R}^d$, regarding the computational cost and the discriminative property, we want to produce a compact features in which the variance of each variable is maximized, the variables are pairwise uncorrelated, and noise and redundancy is removed. Fortunately, these objectives can be easily accomplished by Principal Component Analysis (PCA).

However, deciding how many PCA component to retain is not a trivial task with high-dimensional data. Obviously, we want to compress data as much as possible for computational benefit and, at the same time, want the compressed data still be well representative for original data. Following \cite{_pca_????}, we choose number of components to retain based on the percentage of variance retained - $(0 \le \gamma \le 1)$. 
\vspace{-0.3em}
\begin{equation}
\label{eq:retained_PCA}
\frac{\sum_{j=1}^D \lambda_j}{\sum_{j=1}^n \lambda_j} \ge \gamma
\end{equation}
Where $\lambda_1, \lambda_2, ..., \lambda_n$ is the eigenvalues (sorted in decreasing order) of the covariance matrix $S = \frac{1}{m}\sum_{i=1}^m (\tilde{x}^{(i)})(\tilde{x}^{(i)})^T$.
The number of retained PCA components $D$ is the smallest value which makes the inequality (\ref{eq:retained_PCA}) satisfied. The compressed features can be obtained by: $X = U^T\tilde{X}$.
% \begin{equation}
% 
% \end{equation}
Where $U$ is the stack the eigenvectors corresponding to the top-$D$ eigenvalues of $S$ in columns.

Furthermore, reducing the data’s dimension can also reduce the complexity of the hypothesis class considered and help avoid overfitting in learning a GMM (Section \ref{ssec:proposed_method_embedding}). Pairwise uncorrelated variables is also a desirable property to avoid ill-condition covariance matrix in fitting GMM. 

% \vspace{-0.5em}
\subsection{Posterior probability as embedding features}
\label{ssec:proposed_method_embedding}
Let $\lambda = \{w_i; \mu_i; \Sigma_i; i = 1...N \}$ the set of optimal parameters of the Gaussian Mixture Model GMM learning from $X = \{ x^{(1)}, x^{(2)}, ..., x^{(m)}\}; x^{(i)} \in \mathbb{R}^D$. Where $w_i$, $\mu_i$ and $\Sigma_i$ denote respectively the weight, mean vector and covariance matrix of the $i$-th Gaussian in $N$ Gaussians of the model.

The posterior probability presents the strength of relationship between a sample $x^{(t)}$ and a Gaussian model $N(\mu_j, \Sigma_j)$.
\begin{equation}
P(x^{(t)}|\mu_j, \Sigma_j)=\frac{\exp(-\frac{1}{2}(x^{(t)}-\mu_j)^T\Sigma_j^{-1}(x^{(t)}-\mu_j))}{(2\pi)^{D/2}|\Sigma_j|^{1/2}}
\end{equation}
where $|.|$ denotes the determinant operator. 

The embedding feature of a sample $x^{(t)}$ is constructed as
\begin{equation}
z^{(t)}=\left[P(x^{(t)}|\mu_j, \Sigma_j); j=1...N \right]
\end{equation}
% \vspace{-1.5em}
% In Fisher Vector encoding \cite{FisherVector_4270291}, the GMM is assumed to consist of Gaussian distributions with diagonal covariance matrices. There are three main reasons behind this assumption. First of all, any distribution can be approximated by a weighted sum of Gaussian distributions with diagonal covariances. Secondly, using diagonal covariances have certain computational advantage over using full covariances. Last but not least, the diagonal covariances is required in formulating the approximated closed form for the Fisher information matrix of a GMM.  

In our proposed method, since we do not have the diagonal constrain on the covariance as in Fisher Vector encoding \cite{FisherVector_4270291}, we decide the use full covariances in the GMM to achieve better mixture models. When using full covariances instead of diagonal covariances, it is possible to increase the likelihood, however there is a risk of overfitting as more parameters added. 
Therefore, in order to make a rational comparison between GMM with full and diagonal covariances, we utilize the Bayesian information criterion (BIC)\cite{BIC_STAN:STAN530} as this criterion reduces the risk of overfitting by introducing the penalty term on the number of parameters.

Specifically, from Fig.\ref{fig:BIC_gap}, we found that with a small $N$, e.g. 16, using full covariances can help to achieve better mixture models under BIC. While at a larger $K$, e.g. 64, the BIC values of GMM with diagonal covariances are more comparable to those of GMM with full covariances. Hence, full covariance is preferable.

\begin{figure}[h]
\centering
\caption{The relative gap between BIC values of GMM with full covariance and GMM with diagonal covariance (using VGG-FC7 4096-D descriptors). A negative gap means that the former one is better under BIC.}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/cifar10-vggfc7_BIC_chart.jpg}
\caption{CIFAR-10 \cite{cifar10_krizhevsky2009learning}}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/labelme-vggfc7_BIC_chart.jpg}
\caption{LabelMe-12-50k \cite{labelme_Uetz_large-scaleobject}}
\end{subfigure}
\label{fig:BIC_gap}
\end{figure}
% One should notice that even though the PCA step make data independent among dimension, there is nothing to guarantee that this independent property is still preserved for any arbitrary subset of data.


% a Bayesian may not only be uncertain about the parameter values, but even about the models themselves.
\vspace{-0.8em}
\subsection{Unsparsifying the embedding features}
\label{ssec:proposed_method_unsparsifying}
% Similar to the finding in It is easy to recognize that the embedding feature $z^{(t)}$ is very sparse

% This algorithm explicitly preserves the similarity between Euclidean and Hamming distances

Similar to the finding in \cite{PN_Perronnin:2010:IFK:1888089.1888101}, we also observed that as the number of Gaussians increases, the embedding features become sparser (Fig. \ref{fig:sparse_chart}). This effect can be easily explained: as the number of Gaussians increases, it is easier for a embedding feature $z^{(t)}$ to fit in a distribution with high probability.

% fewer descriptors $x_t$ are assigned with a significant probability $\gamma_t(i)$ to each Gaussian. 

Additionally, we also observe in Fig. \ref{fig:sparse_chart} that as the more discriminative the original global descriptors $\tilde{x}^{(t)}$ are, the sparser their corresponding embedding features $z^{(t)}$ are. This property is also pretty intuitive as the discrimination of descriptors presents the fact that the descriptors of semantically similar images tends to be closed in the $l2$-space, while those of semantically different images locate away from each others. Consequently, GMM will group the semantically similar descriptors into same clusters with very high confident and leaves the probability of being in other cluster to be infinitesimal.

\begin{figure}[h]
\centering
\caption{Histogram of \textbf{log scale} of embedding features for CIFAR-10  \cite{cifar10_krizhevsky2009learning} dataset using GIST 512-D and VGG-FC7 4096-D descriptors.}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/cifar_sparse_16_chart.jpg}
\caption{$N=16$}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\includegraphics[width=\textwidth]{fig/cifar_sparse_64_chart.jpg}
\caption{$N=64$}
\end{subfigure}
\label{fig:sparse_chart}
\end{figure}

Since the $l2$-distance are poor measures of similarity on sparse vectors, we follow \cite{PN_Perronnin:2010:IFK:1888089.1888101} to ``\textit{unsparsify}'' the embedding features by applying the function (\ref{eq:power_norm}) so that we can keep the $l2$-distance similarity. In fact, the $l2$-distance similarity is desirable as the hashing methods preserve the similarity between Euclidean and Hamming distances 
% \vspace{-0.5em}
\begin{equation}
\label{eq:power_norm}
f(z)=\text{sign}(z)|z|^\alpha
\end{equation}


% In \cite{PN_Perronnin:2010:IFK:1888089.1888101}, Perronnin et al. recommend a reasonable value of $\alpha = 0.5$ for $K = 256$ to "\textit{unsparsifying}" the embedding features. However, with different    




==> tex/3-evaluation_3-visualize.tex <==
\subsection{Visualize descriptors}
\label{ssec:visualize_desc}

We utilize t-SNE \cite{t-sne_van2008visualizing} to visualize (Fig. \ref{fig:mnist_cluster}) the scatter plot of GIST 512-D descriptor of a subset of MNIST dataset. We can easily recognize that after processing with Gemb with different number of Gaussians (Fig. \ref{fig:gemb_32}, \ref{fig:gemb_64}), the descriptors of the same classes locate in denser regions and there are also clearer boundaries between different classes. These mean that Gemb is capable of producing more discriminative features.

\begin{figure}[h]
\centering
\caption{Visualizing GIST descriptors of a subset of MNIST dataset. Different colors correspond to different classes. Best viewed in color.}
\begin{subfigure}[b]{0.156\textwidth}
\includegraphics[width=\textwidth]{fig/t-SNE_mnist_raw.jpg}
\caption{Without Gemb}
\end{subfigure}
\begin{subfigure}[b]{0.156\textwidth}
\includegraphics[width=\textwidth]{fig/t-SNE_mnist_emb_32.jpg}
\caption{Gemb ($N=32$)}
\label{fig:gemb_32}
\end{subfigure}
\begin{subfigure}[b]{0.156\textwidth}
\includegraphics[width=\textwidth]{fig/t-SNE_mnist_emb_64.jpg}
\caption{Gemb ($N=64$)}
\label{fig:gemb_64}
\end{subfigure}
\label{fig:mnist_cluster}
\end{figure}
